On the Relationship Between Several Variants of the Linear Hashing Conjecture

In Linear Hashing ($\mathsf{LH}$) with $\beta$ bins on a size $u$ universe ${\mathcal{U}=\{0,1,\ldots, u-1\}}$, items $\{x_1,x_2,\ldots, x_n\}\subset \mathcal{U}$ are placed in bins by the hash function $$x_i\mapsto (ax_i+b)\mod p \mod \beta$$ for some prime $p\in [u,2u]$ and randomly chosen integers $a,b \in [1,p]$. The "maxload" of $\mathsf{LH}$ is the number of items assigned to the fullest bin. Expected maxload for a worst-case set of items is a natural measure of how well $\mathsf{LH}$ distributes items amongst the bins. Fix $\beta=n$. Despite $\mathsf{LH}$'s simplicity, bounding $\mathsf{LH}$'s worst-case maxload is extremely challenging. It is well-known that on random inputs $\mathsf{LH}$ achieves maxload $\Omega\left(\frac{\log n}{\log\log n}\right)$; this is currently the best lower bound for $\mathsf{LH}$'s expected maxload. Recently Knudsen established an upper bound of $\widetilde{O}(n^{1 / 3})$. The question "Is the worst-case expected maxload of $\mathsf{LH}$ $n^{o(1)}$?" is one of the most basic open problems in discrete math. In this paper we propose a set of intermediate open questions to help researchers make progress on this problem. We establish the relationship between these intermediate open questions and make some partial progress on them.

==> abstract.tex <==
In Linear Hashing ($\mathsf{LH}$) with $\beta$ bins on a size
$u$ universe ${\mathcal{U}=\{0,1,\ldots, u-1\}}$, items
$\{x_1,x_2,\ldots, x_n\}\subset \mathcal{U}$ are placed in
bins by the hash function
$$x_i\mapsto (ax_i+b)\mod p \mod \beta$$ 
for some prime $p\in [u,2u]$ and randomly chosen
integers $a,b \in [1,p]$. The "maxload" of $\mathsf{LH}$ is the
number of items assigned to the fullest bin. Expected maxload for
a worst-case set of items is a natural measure of how well $\mathsf{LH}$
distributes items amongst the bins.

Fix $\beta=n$. Despite $\mathsf{LH}$'s simplicity, bounding $\mathsf{LH}$'s worst-case
maxload is extremely challenging. 
It is well-known that on random inputs $\mathsf{LH}$ achieves
maxload $\Omega\left(\frac{\log n}{\log\log n}\right)$; this is
currently the best lower bound for $\mathsf{LH}$'s expected maxload.
Recently Knudsen established an upper bound of
$\widetilde{O}(n^{1 / 3})$. 
The question "Is the worst-case expected maxload of $\mathsf{LH}$
$n^{o(1)}$?" is one of the most basic open problems in discrete
math.

In this paper we propose a set of intermediate open questions to
help researchers make progress on this problem. 
We establish the relationship between these intermediate open
questions and make some partial progress on them.


==> pwiseindep2bins.tex <==
\section{Pairwise Independent $\LH$ for $2$ bins}\label{sec:pairwiseindep2}
In \defn{Uniform Two Bin} $\LH$ ($\ULH$) we hash
$x\in [p]$ via functions parameterized
by $a\in \pnozero,b\in[p]$ defined as 
$$h_{a,b}(x) = \floor{\frac{\posmod_p(ax+b)}{p/2}} \in \set{0,1}.$$

\begin{prop}
  \label{prop:pairwise_concentrate}
  $\ULH$ has expected maxload at most
  $$n/2+\sqrt{n/2}.$$
\end{prop}
\begin{proof}
We say that $x,y\in X$ \defn{collide} if they hash to the same
bin. Let random variable $C$ denote the number of collisions, and
random variable $M$ denote the maxload.
The bins to which distinct $x,y\in X$ map to under $\ULH$
are pairwise-independent, so 
\begin{equation}\label{eq:lhs7ez}
  \E[C] = \frac{1}{2}\binom{n}{2}.
\end{equation}
On the other hand
\begin{equation}\label{eq:rhs7ez}
  \E[C\mid M=m] = \binom{m}{2}+\binom{n-m}{2}.
\end{equation}
Observe that \eqref{eq:rhs7ez} is a quadratic in $m$, and in
particular convex as a function of $m$.
Combining \eqref{eq:lhs7ez},\eqref{eq:rhs7ez} and applying
Jensen's Inequality gives:
\begin{align}
  \frac{1}{2} \binom{n}{2}&\ge
  \E\left[\binom{M}{2}+\binom{n-M}{2}\right]\label{eq:RHSthing}\\
                  &\ge
                  \binom{\E[M]}{2}+\binom{n-\E[M]}{2}\label{eq:jensen}.
\end{align}
Let $\mu$ denote $\E[M]$. 
Simplifying \cref{eq:jensen} gives
$$\mu^2-\mu n+n^2/4-n/2\le 0.$$
Applying the quadratic formula gives
$$\mu \le n/2  + \sqrt{n/2}.$$
\end{proof}

